A Proof of the Schr\"oder-Bernstein Theorem in ACL2

The Schr\"oder-Bernstein theorem states that, for any two sets P and Q, if there exists an injection from P to Q and an injection from Q to P, then there must exist a bijection between the two sets. Classically, it follows that the ordering of the cardinal numbers is antisymmetric. We describe a formulation and verification of the Schr\"oder-Bernstein theorem in ACL2 following a well-known proof, introducing a theory of chains to define a non-computable witness.

==> eptcsdata.tex <==
\providecommand{\firstpage}{36}
\providecommand{\publicationstatus}{Gamboa and Manolios (Eds):\\
ACL2 Workshop 2025\\
EPTCS 423, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.423.3}{10.4204/EPTCS.423.3}}
\pdfoutput=1

